The intriguing role of module criticality in the generalization of deep networks

We study the phenomenon that some modules of deep neural networks (DNNs) are more critical than others. Meaning that rewinding their parameter values back to initialization, while keeping other modules fixed at the trained parameters, results in a large drop in the network's performance. Our analysis reveals interesting properties of the loss landscape which leads us to propose a complexity measure, called module criticality, based on the shape of the valleys that connects the initial and final values of the module parameters. We formulate how generalization relates to the module criticality, and show that this measure is able to explain the superior generalization performance of some architectures over others, whereas earlier measures fail to do so.

==> approximation.tex <==
Given a standard ResNet module with skip connections and parallel modules, we would like to understand the contribution of each path to the final function value.  Let $f(x) \in \mathbb{R}^k$ be the $k$-class output of the neural network, the function $v(\cdot)$ be the input to the ResNet module of interest and the function $g(\cdot)$ represents the function computed by the modules following the current ResNet module. Let $S(\cdot)$ refer to the skip connection function and $h(\cdot)$ be the parallel module to the skip connection.  We can write $f(x)$ as follows,
\begin{align}\label{eq:resnetmodule}
    f(x) = g\left(\underbrace{S(v(x))+h(v(x)}_{\text{`Resnet Module'}})\right).
\end{align}
For the modules where the skip connection is the identity map, $S(\cdot)$ will be an identity matrix of appropriate dimension. In other cases $S(\cdot)$ might a convolutional matrix with appropriate dimensions to downsample the input. This ResNet module has two \emph{paths} along which contributes to the final function being computed. The first is the skip path where $v(x) \mapsto S(v(x))$, the second path is where $v(x) \mapsto h(v(x))$. For a concrete example, let us consider the case when the function $h$ is computed by two fully connected layers with weights $W_1$ and $W_2$, %(this is for the sake of intuition, in general we could have an arbitrary number of fully connected or convolutional layers). 
%Specifically we have,
\begin{align*}
    h(x) = W_2 \sigma(W_1 x).
\end{align*}
and we have ReLU activation. Therefore, the function $f$ is piece-wise linear. Consider a linearization of this function with respect to this ResNet module. If $v(x) \in \mathbb{R}^m$ then for any input $x$, we have that
\begin{align*}
    f_i(x) & = \langle \nabla_S f_i(x),S \rangle + \langle \nabla_{W_2} f_i(x),W_2\rangle \qquad \forall i \in \{ 1,\ldots,k\}\\
    & = \langle \nabla_S f_i(x),S \rangle  + \langle \nabla_{W_1} f_i(x),W_1\rangle \qquad \forall i \in \{ 1,\ldots,k\}.
\end{align*}
% Note that the equality holds as the non-linearity that we are considering is the ReLU function that ensures the function being computed is piecewise linear. 
\note{NC: Need to motivate why each term corresponds to the importance of the path.}

